A Concise Guide on the Integration of Battery Electric Buses into Urban Bus Networks

With the increasing market penetration of battery-electric buses into urban bus networks, practitioners face many novel planning problems. As a result, the interest in optimization-based decision-making for these planning problems increases but practitioners' requirements on planning solutions and current academic approaches often diverge. Against this background, this survey aims to provide a concise guide on optimization-based planning approaches for integrating battery-electric buses into urban bus networks for both practitioners and academics. First, we derive practitioners' requirements for integrating battery-electric buses from state-of-the-art specifications, project reports, and expert knowledge. Second, we analyze whether existing optimization-based planning models fulfill these practitioners' requirements. Based on this analysis, we carve out the existing gap between practice and research and discuss how to address these in future research.

==> figures/figLocations/tabLocations.tex <==
depot&\citealt{Islam2019a}, \citealt{Ke2016a}, \citealt{Lin2019b}\\&
\citealt{Rogge2018a}, \citealt{Tang2019a}, \citealt{Teng2020a}\\&
\citealt{Yao2020a}\\
terminals&\citealt{Dirks2021a}, \citealt{Janovec2019a}, \citealt{Jefferies2020a}\\&
\citealt{Kunith2016a}, \citealt{Kunith2017b}, \citealt{Li2018a}\\&
\citealt{Liu2020a}, \citealt{Lotfi2020a}, \citealt{Paul2014a}\\&
\citealt{Reuer2015a}, \citealt{Rinaldi2019a}, \citealt{Rinaldi2019b}\\&
\citealt{Sassi2017a}, \citealt{Wei2018a}, \citealt{Zhou2020b}\\&
\\
stops&\citealt{Berthold2017a}, \citealt{Chen2013a}, \citealt{Kunith2013a}\\&
\citealt{Liu2018b}, \citealt{Pelletier2019a}, \citealt{Rohrbeck2018a}\\&
\citealt{Sebastiani2016a}, \citealt{Wehres2016a}, \citealt{Xylia2017a}\\&
\citealt{Xylia2017b}\\
stations&\citealt{Adler2017a}, \citealt{An2020a}, \citealt{Li2018c}\\&
\citealt{Li2019a}, \citealt{Lin2019a}, \citealt{Wen2016a}\\&
\citealt{vanKootenNiekerk2017a}\\
swapping&\citealt{An2019a}, \citealt{Li2014a}\\


==> meta/abstract.tex <==
\begin{abstract}
	\new{In this paper we provide a concise guide to the integration of battery electric buses into urban bus networks for practice and research. First, we derive real-world requirements for the integration of battery electric buses from state-of-the-art specifications, project reports and expert knowledge. Second, we analyze the fulfillment of the identified real-world requirements by related prescriptive planning models. Based on this analysis, we identify the gap between practice and research. In particular, we identify neglected real-world requirements and provide insights on how these can be addressed in future research projects.}
%	and we derive real-world requirements for the integration of battery electric buses and identify the gap between practice and research.
%	battery electric bus planning models for battery electric buses integrating 
	
%	we identify the gap between practice and research regarding the planning for the integration of battery electric buses into existing bus networks \new{[MS: We focus on X,Y in particular on the gap between...]}. First, we derive practical requirements from specifications of state-of-the-art battery electric buses, project reports and expert knowledge that are relevant for real-world planning problems. Based on these requirements, we analyze prescriptive planning models within scientific literature regarding the fulfillment of the identified requirements as well as methodological aspects. Based on our analysis, we derive promising research perspectives.
	\begin{keyword}
		battery electric buses;
		planning models;
		survey.
	\end{keyword}
\end{abstract}






==> table/table_1.tex <==
T1&\citealt{Rogge2018a}, \citealt{Liu2020a}, \citealt{Janovec2019a}, \citealt{Ke2016a}, \citealt{Islam2019a}, \citealt{Adler2017a}, \citealt{vanKootenNiekerk2017a}, \citealt{Teng2020a}, \citealt{An2020a}, \citealt{Li2019a}, \citealt{Tang2019a}, \citealt{Yao2020a}, \citealt{Wen2016a}, \citealt{Li2018c}, \citealt{Li2018a}, \citealt{Reuer2015a}, \citealt{Wei2018a}, \citealt{Pelletier2019a}\\
T2&\citealt{Rogge2018a}, \citealt{Janovec2019a}, \citealt{Ke2016a}, \citealt{Islam2019a}, \citealt{Wehres2016a}, \citealt{Kunith2017b}, \citealt{Li2019a}, \citealt{Chen2013a}, \citealt{Liu2018b}, \citealt{Rohrbeck2018a}, \citealt{Yao2020a}, \citealt{Li2018c}\\
T3&\citealt{An2019a}, \citealt{Sebastiani2016a}, \citealt{Rogge2018a}, \citealt{Liu2020a}, \citealt{Ke2016a}, \citealt{Islam2019a}, \citealt{Wehres2016a}, \citealt{Xylia2017a}, \citealt{Lin2019b}, \citealt{Lin2019a}, \citealt{Berthold2017a}, \citealt{Kunith2013a}, \citealt{Kunith2017b}, \citealt{An2020a}, \citealt{Li2019a}, \citealt{Xylia2017b}, \citealt{Chen2013a}, \citealt{Liu2018b}, \citealt{Rohrbeck2018a}, \citealt{Yao2020a}, \citealt{Li2018c}, \citealt{Wei2018a}, \citealt{Kunith2016a}, \citealt{Pelletier2019a}\\
T4&\citealt{Li2014a}, \citealt{Rogge2018a}, \citealt{Islam2019a}, \citealt{Xylia2017a}, \citealt{Li2019a}, \citealt{Xylia2017b}, \citealt{Li2018c}, \citealt{Pelletier2019a}\\
T5&\citealt{Rogge2018a}, \citealt{Islam2019a}, \citealt{Xylia2017a}, \citealt{Lin2019b}, \citealt{Lin2019a}, \citealt{An2020a}, \citealt{Li2019a}, \citealt{Xylia2017b}, \citealt{Li2018c}\\
T6&\citealt{An2019a}, \citealt{Li2014a}, \citealt{Rogge2018a}, \citealt{Ke2016a}, \citealt{Islam2019a}, \citealt{Adler2017a}, \citealt{vanKootenNiekerk2017a}, \citealt{Xylia2017a}, \citealt{Lin2019b}, \citealt{Lin2019a}, \citealt{Sassi2017a}, \citealt{Teng2020a}, \citealt{An2020a}, \citealt{Li2019a}, \citealt{Xylia2017b}, \citealt{Chen2013a}, \citealt{Tang2019a}, \citealt{Yao2020a}, \citealt{Wen2016a}, \citealt{Li2018c}, \citealt{Li2018a}, \citealt{Paul2014a}, \citealt{Reuer2015a}, \citealt{Rinaldi2019b}, \citealt{Rinaldi2019a}, \citealt{Pelletier2019a}\\
F1&\citealt{Islam2019a}, \citealt{Li2018a}, \citealt{Pelletier2019a}\\
F2&\citealt{Islam2019a}, \citealt{Lin2019b}, \citealt{Rohrbeck2018a}, \citealt{Li2018a}, \citealt{Pelletier2019a}\\
F3&\citealt{An2019a}, \citealt{Rogge2018a}, \citealt{Islam2019a}, \citealt{Xylia2017a}, \citealt{Sassi2017a}, \citealt{An2020a}, \citealt{Li2019a}, \citealt{Xylia2017b}, \citealt{Liu2018b}, \citealt{Li2018c}, \citealt{Li2018a}, \citealt{Paul2014a}, \citealt{Reuer2015a}, \citealt{Rinaldi2019b}, \citealt{Rinaldi2019a}, \citealt{Wei2018a}, \citealt{Pelletier2019a}\\
F4&\citealt{Rogge2018a}, \citealt{Janovec2019a}, \citealt{Ke2016a}, \citealt{Adler2017a}, \citealt{Kunith2017b}, \citealt{Li2019a}, \citealt{Liu2018b}, \citealt{Yao2020a}, \citealt{Li2018c}, \citealt{Pelletier2019a}\\
F5&\citealt{Rogge2018a}, \citealt{Kunith2017b}, \citealt{Teng2020a}, \citealt{Li2019a}, \citealt{Yao2020a}, \citealt{Li2018c}, \citealt{Kunith2016a}, \citealt{Pelletier2019a}\\
I1&\citealt{An2019a}, \citealt{Wehres2016a}, \citealt{Xylia2017a}, \citealt{Xylia2017b}, \citealt{Chen2013a}, \citealt{Liu2018b}, \citealt{Pelletier2019a}\\
I2&\citealt{An2019a}, \citealt{Sebastiani2016a}, \citealt{Wehres2016a}, \citealt{Xylia2017a}, \citealt{Lin2019b}, \citealt{Lin2019a}, \citealt{Berthold2017a}, \citealt{Kunith2013a}, \citealt{Kunith2017b}, \citealt{An2020a}, \citealt{Li2019a}, \citealt{Xylia2017b}, \citealt{Chen2013a}, \citealt{Liu2018b}, \citealt{Rohrbeck2018a}, \citealt{Li2018c}, \citealt{Wei2018a}, \citealt{Kunith2016a}\\
I3&\citealt{Wehres2016a}, \citealt{Xylia2017a}, \citealt{Xylia2017b}, \citealt{Chen2013a}, \citealt{Liu2018b}, \citealt{Pelletier2019a}\\
I4&\citealt{An2019a}, \citealt{Rogge2018a}, \citealt{Ke2016a}, \citealt{Lin2019b}, \citealt{Lin2019a}, \citealt{Kunith2017b}, \citealt{Yao2020a}, \citealt{Wei2018a}, \citealt{Kunith2016a}\\
E1&\citealt{Sebastiani2016a}, \citealt{Rogge2018a}, \citealt{Kunith2013a}, \citealt{Kunith2017b}, \citealt{Tang2019a}, \citealt{Liu2018b}, \citealt{Kunith2016a}\\
E2&\citealt{Rogge2018a}, \citealt{Ke2016a}, \citealt{Li2019a}, \citealt{Liu2018b}, \citealt{Yao2020a}, \citealt{Li2018c}, \citealt{Paul2014a}, \citealt{Pelletier2019a}\\
E3&\citealt{An2019a}, \citealt{Wehres2016a}, \citealt{An2020a}, \citealt{Tang2019a}, \citealt{Liu2018b}\\


==> table/table_2.tex <==
C1&\citealt{Sebastiani2016a}, \citealt{Liu2020a}, \citealt{Janovec2019a}, \citealt{Ke2016a}, \citealt{Wehres2016a}, \citealt{vanKootenNiekerk2017a}, \citealt{Xylia2017a}, \citealt{Berthold2017a}, \citealt{Kunith2013a}, \citealt{Sassi2017a}, \citealt{Kunith2017b}, \citealt{An2020a}, \citealt{Xylia2017b}, \citealt{Chen2013a}, \citealt{Liu2018b}, \citealt{Rohrbeck2018a}, \citealt{Wen2016a}, \citealt{Paul2014a}, \citealt{Kunith2016a}\\
C2&\citealt{Sebastiani2016a}, \citealt{Ke2016a}, \citealt{vanKootenNiekerk2017a}, \citealt{Kunith2013a}, \citealt{Kunith2017b}, \citealt{Li2019a}, \citealt{Li2018c}, \citealt{Kunith2016a}\\
S1&\citealt{Li2014a}, \citealt{Liu2020a}, \citealt{Janovec2019a}, \citealt{Adler2017a}, \citealt{vanKootenNiekerk2017a}, \citealt{Teng2020a}, \citealt{Tang2019a}, \citealt{Wen2016a}, \citealt{Paul2014a}, \citealt{Rinaldi2019b}, \citealt{Rinaldi2019a}\\
S2&\citealt{Li2014a}, \citealt{Rogge2018a}, \citealt{Liu2020a}, \citealt{Janovec2019a}, \citealt{Ke2016a}, \citealt{Adler2017a}, \citealt{vanKootenNiekerk2017a}, \citealt{Sassi2017a}, \citealt{Teng2020a}, \citealt{Li2019a}, \citealt{Tang2019a}, \citealt{Yao2020a}, \citealt{Wen2016a}, \citealt{Li2018c}, \citealt{Li2018a}, \citealt{Paul2014a}, \citealt{Reuer2015a}, \citealt{Rinaldi2019b}, \citealt{Rinaldi2019a}, \citealt{Wei2018a}\\
D1&\citealt{An2019a}, \citealt{Li2014a}, \citealt{Rogge2018a}, \citealt{Liu2020a}, \citealt{Janovec2019a}, \citealt{Ke2016a}, \citealt{Adler2017a}, \citealt{vanKootenNiekerk2017a}, \citealt{Lin2019a}, \citealt{Sassi2017a}, \citealt{Teng2020a}, \citealt{An2020a}, \citealt{Li2019a}, \citealt{Tang2019a}, \citealt{Yao2020a}, \citealt{Wen2016a}, \citealt{Li2018c}, \citealt{Reuer2015a}, \citealt{Wei2018a}\\
D2&\citealt{An2019a}, \citealt{Li2014a}, \citealt{Rogge2018a}, \citealt{Liu2020a}, \citealt{Janovec2019a}, \citealt{Ke2016a}, \citealt{Adler2017a}, \citealt{vanKootenNiekerk2017a}, \citealt{Lin2019a}, \citealt{Teng2020a}, \citealt{An2020a}, \citealt{Li2019a}, \citealt{Tang2019a}, \citealt{Yao2020a}, \citealt{Wen2016a}, \citealt{Li2018c}, \citealt{Reuer2015a}, \citealt{Wei2018a}\\

